HoRStify: Sound Security Analysis of Smart Contracts

The cryptocurrency Ethereum is the most widely used execution platform for smart contracts. Smart contracts are distributed applications, which govern financial assets and, hence, can implement advanced financial instruments, such as decentralized exchanges or autonomous organizations (DAOs). Their financial nature makes smart contracts an attractive attack target, as demonstrated by numerous exploits on popular contracts resulting in financial damage of millions of dollars. This omnipresent attack hazard motivates the need for sound static analysis tools, which assist smart contract developers in eliminating contract vulnerabilities a priori to deployment. Vulnerability assessment that is sound and insightful for EVM contracts is a formidable challenge because contracts execute low-level bytecode in a largely unknown and potentially hostile execution environment. So far, there exists no provably sound automated analyzer that allows for the verification of security properties based on program dependencies, even though prevalent attack classes fall into this category. In this work, we present HoRStify, the first automated analyzer for dependency properties of Ethereum smart contracts based on sound static analysis. HoRStify grounds its soundness proof on a formal proof framework for static program slicing that we instantiate to the semantics of EVM bytecode. We demonstrate that HoRStify is flexible enough to soundly verify the absence of famous attack classes such as timestamp dependency and, at the same time, performant enough to analyze real-world smart contracts.

==> related-work.tex <==
The continuing reports on devastating exploits of smart contract vulnerabilities led to a vast number of works on the automated static analysis of Ethereum smart contracts. 

Most practical static analysis tools focus on the heuristic detection of certain (classes of) smart contract bugs. 
This line of work was pioneered by the static analyzer Oyente~\cite{luu2016making} that supports heuristics for the detection of reentrancy, timestamp dependence, unhandled exceptions, and transaction order dependence bugs. 
Bug finding tools do not strive to provide theoretical guarantees for their analysis approach or the used detection patterns.
Consequently, this line of research differs substantially in aim and scope from the one of our work, and we refer the reader to recent surveys~\cite{GMS::CAV18, di2019survey,liu2019survey} for more details.

To the best of our knowledge, the only tools targeting sound and automated static analyses of smart contract security properties are Securify~\cite{tsankov2018securify}, ZEUS~\cite{kalra2018zeus}, EtherTrust~\cite{GMS::CAV18}, NeuCheck~\cite{lu2019neucheck}, and~\cite{schneidewind2020ethor}. The soundness claims of ZEUS, Securify, EtherTrust, and NeuCheck are systematically confuted in~\cite{schneidewind2020good} and~\cite{schneidewind2020ethor}.
Further, out of those tools, Securify is the only one whose core analysis supports dependence properties.

Even though formally proven sound, the tool eThor only supports the sound analysis of reachability properties. 
Consequently, the dependency properties discussed in this work (foremost, timestamp dependence) fall out of the scope of eThor's analysis.

==> timestamp.tex <==
\begin{definition}[Timestamp dependency pattern]
    \label{app:prop:timestamp}
    The timestamp dependency pattern $\pattime$ of a contract $\precontract$ is defined as follows:
    
    \noindent {\small
        \begin{align*}
            \pattime \define
            &\{  \pred{InstMayDepOn}(\lpc, \envvar{\TIMESTAMP}) 
            ~|~ \precontract(\lpc) = (\CALL(\vec{x}, \nextpc, \pre))
            \} \\
            &\cup 
            \{  \pred{VarMayDepOn}(x_i, \envvar{\TIMESTAMP}) 
            ~|~ \precontract(\lpc) = (\CALL(\vec{x}, \nextpc, \pre)~\land~ 0 < i \leq 7)
            \}
        \end{align*}
    }
    which is matched by the contract $\precontract$ if $\forall p.~ p\in \pat(\precontract).~ p \not \in \lfp{\rules{\precontract}}$.
\end{definition}

\begin{definition}[Semantic Timestamp Independence]
    \label{app:prop:timestamp-sem}
    Semantic Timestamp Independence (denoted $\pattimesem$) of a contract $\precontract$ is defined as follows:
    
    \noindent {\small
        \begin{align*}
            \pattimesem \define
            &\{  \iio(\lpc, \envvar{\TIMESTAMP}) 
            ~|~ \precontract(\lpc) = (\CALL(\vec{x}, \nextpc, \pre))
            \} \\
            &\cup 
            \{  \vio(x_i, \envvar{\TIMESTAMP}) 
            ~|~ \precontract(\lpc) = (\CALL(\vec{x}, \nextpc, \pre)~\land~ 0 < i \leq 7)
            \}
        \end{align*}
    }
    which holds for the contract $\precontract$ if all independence predicates $p\in \pattimesem$ hold.
\end{definition}

\begin{definition}[Independence of the block timestamp]
    A contract $C$ is independent of the block timestamp if for all reachable configurations $(\transenv, \cons{\annotate{s}{C}}{\callstack})$ it holds for all $\transenv'$ that 
    \vspace{-0.2cm}
    \noindent
    {\small
        \begin{align*}
            \transenv \equalupto{\timestamp} \transenv' 
            ~\land \sstepstrace{\transenv}{\cons{\annotate{\exstate}{C}}{\callstack}}{\cons{\annotate{\exstate'}{C}}{\callstack}}{\pi}
            ~\land~\finalstate{\exstate'} \\
            \land~ \sstepstrace{\transenv'}{\cons{\annotate{\exstate}{c}}{\callstack}}{\cons{\annotate{\exstate''}{C}}{\callstack}}{\pi'} ~\land~ \finalstate{\exstate''} 
            \implies \project{\pi}{\filtercallscreates{C}} = \project{\pi'}{\filtercallscreates{C}}
    \end{align*}}
    \vspace{-0.5cm}
\end{definition}


\begin{theorem}[Soundness of the timestamp dependence pattern]
    Let $C$ be a contract and $\precontract$ be a contract with sound preprocessing information that is consistent with $C$. 
    If $\precontract$ matches the pattern $\pattime$ then $C$ is timestamp independent.
\end{theorem}

%The \textsf{timestamp dependency} pattern (Definition \ref{prop:timestamp}) implies that all \inst{call} instructions and their used variables are independent of the \inst{timestamp}.
%We have two paths to the \textit{exit} node that start in equal states up to the \inst{timestamp} as premise and want to conclude that they have the same call traces.
%The foundation of the proof is to map the \textsf{timestamp dependency} pattern to a semantic pattern with the independence correctness results and \textbf{InstIndOf} and \textbf{VarIndOf}.
%After that, we cut the two paths into pieces that start and end at defining nodes of the variables that a \inst{call} uses.
%We show that these cut paths have the same \inst{call} traces and the same ordering of \inst{calls}.
%Finally, we argue that the arguments of \inst{calls} have the same values. 
\newcounter{tsproof}
\begin{proof}
    Let $C$ be a contract and $\precontract$ be a contract with sound preprocessing information that is consistent with $C$. 
    We assume that $\precontract$ matches $\pattime$ and show that $\project{\as}{\filtercallscreates{c}} = \project{as'}{\filtercallscreates{c}} $
    We have two executions from node $n$ to the $\exit$ that starts in states $\cfgstate_1$ and $\cfgstate_2$ with $(1) ~\cfgstate_1 \equalupto{\ts} \cfgstate_2$.
    Let 
    $$(2) ~ \conf{n}{\cfgstate_1} \xrightarrow{\as}^*~ \conf{\exit}{\_} 
    \quad \text{and} \quad
    (3) ~ \conf{n}{\cfgstate_2} \xrightarrow{\as'}^*~ \conf{\exit}{\_}$$ be these two executions with path $\as$ and $\as'$.
    \\
    With the correctness \Cref{app:thm:soundness-independence,thm:inst-soundness-independence} and $\pattime$ we have the semantic version of the timestamp dependence pattern $(4) ~ \pattimesem$.
    The proof has two identical directions.
    We show that $\projectpath{\as}{\filtercallscreates{}} ~\odss~ \projectpath{\as'}{\filtercallscreates{}}$.
    Let $\cvar$ be the set of all variables used in calls:
    $$(5) ~\cvar = \{x_i ~ \mid ~  (\CALL(\vec{x}, \nextpc, \pre)) \in \as ~\land~ 0 < i \leq 7\}$$
    Let $X$ be a variable from $\cvar$ and $X \in \vio(X,\inst{timestamp})$ by \pattimesem. 
    The semantic predicate $\vio(X,\inst{timestamp})$ ensures that all writes to variable $X$ in path $\as$ also happen in path $\as'$. 
    Now, we split $\as$ and $\as'$ in subpaths starting/ending at nodes where $X$ is defined.
    We then argue that these split parts have the same call traces; this is enough to show that paths $\as$ and $\as'$ have the same call traces. \\
    Let $as_i$ and $as_i'$ be such paths%
    \footnote{We omitted to let the last split paths of $\as/\as'$ end at the \textit{exit} node although this border case is formally required.}
    outgoing from the $i$-th $X$ definition:
    $$ (6)
    ~~~\conf{n}{\cfgstate_1} \nstep{}{}{N_X}{i} \conf{n_X}{\cfgstate_1'} \nstep{\as_i}{}{N_X}{1} \conf{n_X'}{\cfgstate_1''}  
    \qquad
    ~~~\conf{n}{\cfgstate_2} \nstep{}{}{N_X}{i} \conf{n_X}{\cfgstate_2'} \nstep{\as_i'}{}{N_X}{1} \conf{n_X'}{\cfgstate_2''}  $$
    We now show that
    $$ (7)~ \projectpatheqlength{as_i}{\as_i'}{n^{\textit{call}}} $$
    holds for all nodes $n^{\textit{call}}$ identifying call instructions. That is, all split paths in $\as$ and $\as'$ visit $n^{\textit{call}}$ the same number of times.
    By $\iio(n^{\textit{call}},\inst{ts})$ instantiating with (1), we have that for all executions
    $$ (*)~~ \conf{n}{\cfgstate_1} \nstep{\textit{xs}}{}{\{n_X'\}}{i} \conf{n_X'}{\hat{\cfgstate_1}} \text{ and } 
    \conf{n}{\cfgstate_2} \nstep{\textit{ys}}{}{\{n_X'\}}{i} \conf{n_X'}{\hat{\cfgstate_2}}$$
    it follows 
    $$ \projectpatheqlength{\textit{xs}}{\textit{ys}}{n^{\textit{call}}} $$
    Premise $(*)$ can be instantiated with every $n_X' \in N_X$ and iterated for every $i$ with (6.1) and (6.2).
    Thereby we have 
    $$ (**)~~ \forall~i.~ \projectpatheqlength{\sum_{0}^{i} \as_i}{\sum_{0}^{i} \as_i'}{n^{\textit{call}}}$$
    Statement (7) follows with $(**)$ and definition of paths $\as_i$ and $\as_i'$ in (6).
    It states that all corresponding split paths visit a call instruction $n^{\textit{call}}$ the same number of times.
    We left to argue that the ordering of the types of \inst{call} instruction is the same since 
    $$ \as_i = [\textit{call}_0(b), \textit{delegatecall}_1(b)]\qquad \as_i' = [\textit{delegatecall}_1(b), \textit{call}_0(b)] \qquad  \lightning$$
    would be different call traces. 
    Those traces can be rejected by instantiation node $n_X'$ in $(*)$ with calls and check the number of appearances (i.e.\ counting of $n^{\textit{call}}$) of the other \inst{call} nodes.
    For example, with
    $$
    n_X' = \textit{call}_0(\cdot) \quad \text{ and } \quad n = \textit{delegatecall}_1(\cdot)
    $$
    we can infer whether $\textit{call}_0(\cdot)$ and $\textit{delegatecall}_1(\cdot)$ appear in the same order in both paths.
    Therefore, (8) all corresponding paths visit every call instruction in the same order and quantity.
    
    It is left to show that corresponding calls have the same values as arguments. 
    With $\vio(X,\pred{timestamp})$ for all used variables in calls, we can conclude that the variables have to be equal.
    Since all used variables at the \inst{call} instructions are equal, (9) the whole usage sets agree at all \inst{call} instructions.
    From (7), (8) and (9) it follows that $\projectpath{\as}{\filtercallscreates{}} ~\subseteq_{od}~ \projectpath{\as'}{\filtercallscreates{}}$ because all \inst{calls} in path $\as$ are in the same ordering and have the same arguments as in path $\as'$.
    
    To conclude that both parts are identical, the dual ($\projectpath{\as'}{\filtercallscreates{}} ~\subseteq_{od}~ \projectpath{\as}{\filtercallscreates{}}$) follows from the symmetric argument.
\end{proof}

